A Learning Theoretic Perspective on Local Explainability

In this paper, we explore connections between interpretable machine learning and learning theory through the lens of local approximation explanations. First, we tackle the traditional problem of performance generalization and bound the test-time accuracy of a model using a notion of how locally explainable it is. Second, we explore the novel problem of explanation generalization which is an important concern for a growing class of finite sample-based local approximation explanations. Finally, we validate our theoretical results empirically and show that they reflect what can be seen in practice.

==> sections/old-intro.tex <==
In practical applications of machine learning, there has been a growing emphasis on the interpretability of learned models for effective and safe deployment. However, despite frequent references to an ``accuracy interpretability trade-off'' in recent interpretability literature, formal connections between learning theory and interpretability remain relatively unstudied. 
That a meaningful relationship would exist between these areas is fairly intuitive. 
For supervised learning, learning theoretic results have thoroughly explored relationships between \textit{generalization} and a function class's \textit{complexity}. 
Additionally, it would be generally uncontroversial to posit that there exists a trade-off between a model's complexity and general notions of its \textit{interpretability}. 
Thus, the complexity of a function's shape should naturally link generalization and interpretability. 
However, the key challenge lies in formalizing these relationships meaningfully. 

The only prior work in the intersection of learning theory and interpretability explored the relationship between the test performance of $f$ on task $(x,y) \sim D$ and how closely $f$ can be \textit{globally} approximated by a function from an interpretable class \cite{Semenova2019Rashomon}.
While global explanations are one way to convey interpretability, another common and flexible approach is to use local explanations.  
Formally, local explanations provide insight into a model's behavior as follows: for any black-box model $f \in \mathcal{F}$ and input $x$, the explanation system produces a simple local approximation $g_x(x') \in \Glocal$ which fits to $f$ in a specified neighborhood $x' \sim N_x$. 
Crucially, the freedom to specify both $\Glocal$ and $N_x$ grants local explanations great versatility for explaining various $f$. 
In this paper, we provide two connections between learning theory and \textit{local} explainability. 

For our first result, in a similar vein to \cite{Semenova2019Rashomon}, we study \textit{performance generalization}, relating  test performance to a notion of  interpretability. As it turns out, our focus on local explanations leads us to completely different tools and insights for this more flexible setting. Our second result identifies and answers an unstudied -- yet important -- question regarding \textit{explanation generalization}. This question stems from our observation regarding a growing class of explanation systems, such as MAPLE \citep{Plumb2018MAPLE} and RL-LIM \citep{Yoon2019}, which aim to leverage the structure of the data distribution $D$ while generating local explanations. Specifically, as these approaches learn their local models using a common finite sample drawn from $D$, they can run the risk of overfitting their explanations to this sample. In light of this, we ask: for these classes of \textit{sample-based} explanation-learning algorithms, how well do the explanations generalize to data not seen during training? 

%Unfortunately, what grants local explanations their versatility also renders their linkage to generalization technically challenging. From a learning-theoretic point of view, the main difficulty here is in being able to quantify the (Rademacher) complexity of the \textit{explanation system}, which is the ensemble of infinitely many locally approximations $\{g_{x'} | x' \in \mathcal{X}\}$ -- this ensemble is far more complex than simpler counterparts that could be used to locally \greg{globally?} approximate $f$, like piecewise models. From an interpretability point of view, an additional subtlety is that the very notion of local explainability is heavily mediated by choices of $N_x$. In regards to performance generalization, one can always specify $N_x$ to degenerately be a point mass at each $x$, thereby allowing one to obtain ``perfect local explainability'' any $f$ (i.e. simply by setting $g_x(x') = f(x)$). Since this holds no matter the complexity of $f$, this notion of local interpretability would not be able to provide any meaningful indication of $f$'s generalization. \jeff{is this at all better?}  Intuitively, being interpretable according to wider neighborhoods would provide more  information about $f$'s complexity, and thus generalization, but this effect should ideally be formalized for any $N_x$. \jeff{TODO: Need to think more carefully if there is a clean adaptation/example that pertains to Theorem 2's setting?} \vaish{I know this paragraph is under TODO, but thought this might be useful for you to know: I think the argument ``As such, any result relating ... meaningful relationship'' may not be obvious to the reader who might ask, ``why not? I could still get a bound using such a $g$ and it may depend on the complexity of $\mathcal{F}$. Why is it not meaningful?''}
%\greg{This paragrph reads like a more techinically complicated version of the previous (proposed) paragraph.  I wonder if the simple version goes in the intro and the complex one goes in a later section}
%\ameet{reading this again, I think it could make sense to remove this paragraph entirely from the intro, and instead include some version of this at the beginning of section 4.  I do think we want to mention somewhere that our analysis is non-trivial; maybe we could do this by adding an additional bullet in the list of contributions where we say something about the technical approach being of general interest and explaining at a very high-level (like one sentence) why this is the case? } \vaish{I'm fine with this! Will save space too, I guess.}


%Unfortunately, what grants local explanations their versatility also renders their linkage to generalization technically challenging. That is, local approximations and their corresponding metrics for interpretability are heavily mediated by the choices of $N_x$ and $\Glocal$.  Indeed, one can always specify the two parameters to degenerately deem a function ``perfectly explainable.'' For instance, if $N_x$ is chosen to be a point mass at each $x$, one can set $g_x(x') = f(x)$ to obtain explanations that are consistently faithful on their infinitesimally small neighborhoods. Similarly, the surrogate class could be chosen to be complex enough to contain $f$ itself, leading to an exactly matching global approximation. However, since these scenarios allow for any $f$ to be considered perfectly explainable, it would be impossible for them to provide any indication of $f$'s generalization. \vaish{This ideas here might require some rephrasing e.g., the concept of ``providing unique information'' was unclear to me.} \jeff{Does this seem better?} Intuitively, wider neighborhoods and simpler approximations would provide more meaningful information about $f$. But to preserve flexibility, any results should handle arbitrary choices of the two.


%In this work, we tackle such challenges head-on and are, to the best of our knowledge, the first to obtain results formally relating local interpretability and generalization. \vaish{We already implied that we're the first already, so do we want to keep this?} 
%\vaish{Add introductory line here indicating that now we'll present our two bounds at a high level.}
We now present our two bounds at a high-level. Regarding performance generalization, we derive our first main result, Theorem \ref{thm:performance-generalization}:
\begin{center}
\scalebox{0.90}{$
\underbrace{\vphantom{\frac{1}{m}\sum_{i=1}^m (f(x_i)-y_i)^2}
\mathbb{E}_{(x,y)\sim D}[(f(x)-y)^2]}_{\text{Test MSE}
} \leq  
\mathcal{O}\Big( \underbrace{\frac{1}{m}\sum_{i=1}^m (f(x_i)-y_i)^2}_{ \text{Train MSE}} + 
\underbrace{\vphantom{\frac{1}{m}\sum_{i=1}^m (f(x_i)-y_i)^2}
\mathbb{E}_{\stackunder[0pt]{$\scriptstyle{x\sim D},$}{$\scriptstyle{x' \sim N_{x}}$}}\left[ (g_{x'}(x)-f(x))^2 \right]}_{\text{Interpretability Term ($\mirNF$)}} 
+ 
\underbrace{\vphantom{\frac{1}{m}\sum_{i=1}^m (f(x_i)-y_i)^2}
\rho_S \hat{\mathcal{R}}_S(\Glocal)\ln m}_{\text{Complexity Term}} \Big)
$
}
\end{center}
%I've change \left( to \big( to save space
%\vphantom is to align the brackets


This represents a bound for the expected test MSE of any $f$ in terms of its training loss over the $m$ samples in the training set $S$. In a standard learning theory approach, such a result would involve the training loss and a term that captures the complexity of $\mathcal{F}$. Here, we replace the latter term, by two terms that involve $\mathcal{G}$. %\jeff{@Vaishnavh, in your suggestion you wrote $\mathcal{G}$ but maybe you meant $\Glocal$?}: \vaishnavh{@Jeff: Sorry about the confusion.}
%\vaish{If we want to say this, the reader would expect numerical/theoretical comparisons between neural network bounds and our bounds.} \vaish{As Ameet says, we need to add a disclaimer.} \jeff{is this phrasing still problematic even with a disclaimer (below the two terms)?}  is replaced by the following two terms:

\begin{enumerate}
    \item[(1)] \textit{Interpretability term:} We define Mirrored Neighborhood Fidelity ($\mirNF$), a quantity which we use to measure $f$'s local interpretability. As we explain further in Section \ref{sec:MNF}, this definition reasonably modifies Neighborhood Fidelity ($\NF$), an existing metric, to aid in our theoretical results. However, it also represents a promising new way to formulate local interpretability, as it can be shown to result in unique advantages and practical trade-offs when compared to $\NF$. 
    \item [(2)]\textit{Complexity term:} This term measures the complexity of the local explanation system $g$ in terms of (a) the complexity of the local explanation class $\Glocal$ and (b) $\rho_S$, a quantity that we define and refer to as \emph{neighborhood disjointedness factor}. As we discuss in Section \ref{sec:performance}, $\rho_S$ is a value in $[1,\sqrt{m}]$ (where $m=|S|$) that is proportional to the level of disjointedness of the neighborhoods for points in the sample $S$. Intuitively, we expect $\rho_S$ to be larger when the neighborhoods sizes are smaller since smaller neighborhoods will overlap less. %\vaish{I think it'll be helpful to be more concrete about relationship between $\rho_S$, neighborhood width and neighborhood disjointedness. `` This term measures the complexity of the local explanation system $g$ in terms of (a) the complexity of the local explanation class $\Glocal$ and (b) $\rho_S$, a quantity that we define and refer to as \emph{neighborhood disjointedness factor}. As we discuss in Section \ref{sec:performance}, $\rho_S$ is a value in $[1,\sqrt{m}]$ that is proportional to the level of disjointedness of the neighborhoods for points in the sample $S$. , Intuitively, we expect $\rho_S$ to be larger when the neighborhoods sizes are smaller since smaller neighborhoods are more disjoint/overlap less. ''}
\end{enumerate}

Notably, a key implication of this bound is that if $\mirNF$ and $\rho$ can be jointly controlled, one is able to obtain a bound that depends on $\Glocal$ instead of $\mathcal{F}$, thus granting an additional avenue to possibly help reason about the performance of $f$. Here, the choice of $N_x$ is crucial, as wider neighborhoods will tend to trade off increasing $\mirNF$ (as explanations are required to extrapolate farther) while decreasing $\rho_S$. Since $\hat{\mathcal{R}}_S(\Glocal)$ can be considered to grow at rate $\mathcal{O}(1/\sqrt{m})$, the bound becomes non-trivial if $N_x$ can be chosen such that $\mirNF$ remains small but $\rho_S$ grows slower than $\mathcal{O}(\sqrt{m})$, a fact which we show empirically holds on some UCI regression datasets (see Section \ref{sec:experiments}).

Finally, another notable aspect of our result is that it treats $\mathcal{F}$ as a black-box, and hence the bound would be valuable when reasoning about $\mathcal{F}$ is difficult, such as in neural networks. However, we must clarify that we do not numerically evaluate these bounds for neural networks. Our focus is rather on the theoretical implications of this bound. 

%\vaish{I think beginning this discussion with that disclaimer might be like starting off with the wrong foot. Some alternative ideas: ``Here, we replace the latter term, by two terms that involve $\mathcal{G}$:''.
%\begin{itemize}
%    \item Interpretability term...
%    \item Complexity term...
%\end{itemize}
%A key implication of our result is that if $\mirNF$ ... datasets (see Section \ref{sec:experiments}). 
%}

%From a learning theory point of view, this result explores local interpretability as a new form of bias for deriving generalization results. Potentially, this grants an additional avenue to help explain the strong test performance of models from complex classes (e.g. neural networks), whenever the learned $f$ is locally explainable \vaish{minor: might want to tone this sentence down even further.} \jeff{should we just get rid of this sentence?}. From an interpretability point of view, Theorem 1 can also help reason about more complex methods which leverage \emph{supervised neighborhoods}. In contrast to default approaches, which choose $N_x$ of constant width for all $x$, these methods dynamically specify the neighborhood at each input. Thinking about trading-off the interpretability and informativeness terms allows us to discuss advantages of said methods, as well recommend new approaches. Meanwhile, the same proof technique for Theorem 1 leads to Theorem 2, a bound for an explanation system's expected performance,  which is a key practical unknown for local explanation methods. Theorem 2 is of particular applicability in many supervised neighborhood settings, and more generally whenever task-data is directly used to select neighborhoods. %These methods include not only existing approaches such as RL-LIM \citep{Yoon2019} and MAPLE \citep{Plumb2018MAPLE}, but also the explanation system we derive based on minimizing empirical MNF (see Section \ref{Sec:MNF}). 


For the second question regarding explanation generalization, we apply a similar proof technique to simultaneously obtain Theorem 2, also presented more coarsely as: 
\begin{center}
\scalebox{0.9}{
$
\underbrace{\vphantom{\sum_{i=1}^{m} \mathbb{E}_{x' \sim N_{x}} \left[ (f(x_i)-g_{x'}(x_i))^2\right]}
\mathbb{E}_{\stackunder[0pt]{$\scriptstyle{x\sim D},$}{$\scriptstyle{x' \sim N_{x}}$}}\left[ (g_{x'}(x)-f(x))^2 \right]}_{\text{Test } \mirNF } 
\leq 
\underbrace{\sum_{i=1}^{m} \mathbb{E}_{x' \sim N_{x}} \left[ (f(x_i)-g_{x'}(x_i))^2\right]}_{ \text{Train } \mirNF} + 
\underbrace{\vphantom{\sum_{i=1}^{m} \mathbb{E}_{x' \sim N_{x}} \left[ (f(x_i)-g_{x'}(x_i))^2\right]}
\mathcal{O} \left (\rho \hat{\mathcal{R}}_S(\Glocal)\ln m\right)}_{\text{Complexity Term}}
$
}
\end{center}
As mentioned earlier, this result concerns a setting in which $g$ are learned using a finite sample drawn from the (unknown) data distribution $D$. Notably, this does not pertain to commonly used LIME explanations \citep{Ribeiro2016}, as they do not learn explanations using samples drawn from $D$. However, the setting is relevant for more recent approaches  including MAPLE \citep{Plumb2018MAPLE} and RL-LIM  \citep{Yoon2019} (see Section \ref{sec:explanations} for a more thorough discussion). For such explanation systems, we bound the expected quality of $g$ as measured by its ``test $\mirNF$'' in terms of its ``train $\mirNF$'', which is the biased empirical estimate of $\mirNF$ using the same $S$. The complexity term is the same as for Theorem \ref{thm:performance-generalization}, thereby capturing the same effect for the varying the width of neighborhoods. A key implication here is that if one can increase neighborhood width without sacrificing empirical explanation quality, one can guarantee better explanations on unseen data relative to $\mirNF$. 





We summarize our main contributions as follows:

\begin{itemize}

\item % I changed the first sentence to your suggestion, Vaishnavh.
In order to make theoretical connections between local interpretability and generalization, we first propose $\mirNF$, a novel measure of local interpretability, as a close alternative to $\NF$. As an aside, we note that, from an interpretability practitioner's point of view, our proposed metric $\mirNF$ offers certain important advantages (and also drawbacks) compared to $\NF$ in terms of being able to evaluate and learn explanations. We discuss this briefly in Section \ref{sec:MNF}, where we also present a way to learn explanations using $\mirNF$, while relegating most of these details to Appendix \ref{sec:mnf-appendix}. 

\item We make a novel connection between performance generalization and local interpretability, arriving at Theorem 1, a general bound for the test MSE of any model in terms of its empirical MSE and $\mirNF$. Our proof technique here is of independent theoretical interest as provides a new way to bound the Rademacher complexity of a \textit{randomized} function (more details in Section \ref{sec:performance}).

\item We motivate an important new generalization question about expected explanation quality for a growing class of \textit{sample-based} local explanation algorithms. For this problem, we arrive at Theorem \ref{thm:explanation-generalization}, a bound for test $\mirNF$ in terms of empirical $\mirNF$. 


\item Through instantiating our general result on UCI Regression datasets, we argue that our result non-trivially reflects the two types of generalization in practice. Specifically, we demonstrate that $\rho$'s growth rate can be made to be smaller than $\mathcal{O}(\sqrt{m})$ without significantly increasing the $\mirNF$ terms. Additionally, for Theorem \ref{thm:explanation-generalization}, we also show experiments demonstrating that the generalization gap empirically improves with larger neighborhoods. 
\end{itemize}


%\vaish{
%We summarize our main contributions as follows: 
%\begin{itemize}
%\item We propose MNF, a novel measure of local interpretability, that is a reasonable alternative to NF which allows us to theoretically study local interpretability. As an aside, we note that, from an interpretability practitioner's point of view our proposed metric MNF offers certain important advantages (and also drawbacks) compared to NF in terms of being able to evaluate explanations and learn explanations. We discuss this briefly in Sec. blah, where we also present a way to learn explanations using MNF, while relegating most of these details to the appendix blah. (and in Sec blah actually make a mention of the explanation learning algorithm.)

%\item We make a novel connection between performance generalization and local interpretability, arriving at Theorem 1, a general bound for the test MSE of any model in terms of its empirical MSE and $\mirNF$. Our proof technique here is of independent theoretical interest as provides a new way to bound the Rademacher complexity of a \textit{randomized} function (more details in Section blah).

%\item We motivate an important new generalization question about expected explanation quality for a growing class of \textit{sample-based} local explanation algorithms. For this problem, we arrive at Theorem \ref{thm:explanation-generalization}, a bound for test $\mirNF$ in terms of empirical $\mirNF$. 

%\item Through instantiating our general result on UCI Regression datasets, we argue that our result non-trivially reflects the two types of generalization in practice. Specifically, we demonstrate that $\rho$'s growth rate can be made to be smaller than $\mathcal{O}(\sqrt{m})$ without significantly increasing the $\mirNF$ terms. For Theorem \ref{thm:explanation-generalization}, we also show \jeff{TODO: Experiments showing bound empirically improving with larger neighborhoods for Theorem 2}

%\item (if the first line is too long, can do this instead) Finally, from an interpretability practitioner's point of view, we note that our proposed metric MNF offers certain important advantages (and also drawbacks) compared to NF in terms of being able to evaluate explanations and learn explanations. We discuss this briefly in Sec. blah, where we also present a way to learn explanations using MNF, while relegating most of these details to the appendix blah. (and in Sec blah actually make a mention of the explanation learning algorithm.)
%\end{itemize}

%}



%one broad form of understanding a model's behavior is to be able to approximate it with one or many simpler functions. In particular, such approaches fall into two general classes: methods which are \emph{by-design globally interpretable}
%and methods which produce \textit{post-hoc local explanations} \greg{This categorization does not seem accurate.  Do we need to define global approximations for our method to make sense?  My guess is that we don't.}. \vaish{I think this is just to provide a more holistic context?} More formally, the former try to directly learn a model $f$ from a class of functions $\mathcal{F}$ deemed to be interpretable. Meanwhile, the latter selects any $\mathcal{F}$ but for each input $x$, produces a simple local approximation $g_x(x')$ which fits to $f$ in a specified neighborhood $x' \sim N_x$.

%\begin{enumerate}
%   \item[(1)] How well can one expect $f$ to perform?
%   \item[(2)] How (locally) interpretable can one expect their model to be? For approximation-based explanations, this is a question of how faithful one can expect their explanations to be.
%  \item[(3)] Given that neither performance nor (local) interpretability is sufficient on its own, to what extent can one characterize their relationship? 
%\end{enumerate}


%\jeff{Does this paragraph add enough to keep here? Or does it detract from the focus?} \greg{up to this point and based on what I remember of the results, I'm not sure why we need to talk about Global Approximation.  Is this just for comparing to the Rashomon work?} For methods that are by-design globally interpretable, corresponding questions are more straightforward to answer. As all interpretability concerns are enveloped by the the choice of $\mathcal{F}$, (2) is addressed by default. Further, any individual method is effectively a single supervised learning problem. Thus, (1) can be addressed directly by standard learning theory and (3) simply involves comparing the results of multiple such analyses (across different choices of $\mathcal{F}$).

%However, not all tasks can be adequately solved by globally interpretable models \com{TODO: Citations/examples needed?}. \greg{Global approxiamtion quality is directly linked to accuracy.  That's their main limitation} But unlike by-design methods, local explanations jointly involve three separate components: a model, a set of local explanations, and a particular choice of neighborhoods \vaish{minor: might want to remind reader what ``neighborhoods'' mean.}. Because of this, answering the same three core questions above becomes more technically challenging.

%\begin{enumerate}
%    \item[(1)] While standard learning theoretic results could be used to analyze $\mathcal{F}$ alone, current approaches remain limited in their applicability. For popular “black-box” model classes, such as neural networks, it has proved difficult to obtain theoretical results which adequately match up to the strong test performance seen in practice. 
%    \item[(2)] Since unique explanations are generated for each possible $x$, local faithfulness can differ greatly depending on the locality in the input space one is trying to explain. It is not possible to enumerate all possible centering points, so we ideally want an overall metric for how well the model can be locally approximated around task-relevant but unseen points.
%    \item[(3)] Local approximations and  their corresponding metrics for interpretability are heavily mediated by the choices of neighborhood and the local surrogate class. For instance, one can degenerately achieve ``perfect explanations'' for any $f$ by defining $N_x$ as a point mass at $x$ and fitting $g_x(x') = f(x)$. Similarly, one could also define the surrogate class to be $\mathcal{F}$ and fit an exactly matching global approximation. Intuitively, being interpretable over wider neighborhoods and using simpler  surrogates would provide more meaningful information about $f$. But to preserve the useful flexibility of local explanations, any results should ideally handle arbitrary choices of the two.
%\end{enumerate}
